Observational constraints on the origin of the elements. I. 3D NLTE formation of Mn lines in late-type stars

Manganese (Mn) is a key Fe-group elements, commonly employed in stellar population and nucleosynthesis studies to explore the role of SN Ia. We have developed a new non-local thermodynamic equilibrium (NLTE) model of Mn, including new photo-ionisation cross-sections and new transition rates caused by collisions with H and H- atoms. We applied the model in combination with 1-dimensional (1D) LTE model atmospheres and 3D hydrodynamical simulations of stellar convection to quantify the impact of NLTE and convection on the line formation. We show that the effects of NLTE are present in Mn I and, to a lesser degree, in Mn II lines, and these increase with metallicity and with effective temperature of a model. Employing 3D NLTE radiative transfer, we derive new abundance of Mn in the Sun, A(Mn)=5.52 +/- 0.03 dex, consistent with the element abundance in C I meteorites. We also apply our methods to the analysis of three metal-poor benchmark stars. We find that 3D NLTE abundances are significantly higher than 1D LTE. For dwarfs, the differences between 1D NLTE and 3D NLTE abundances are typically within 0.15 dex, however, the effects are much larger in the atmospheres of giants owing to their more vigorous convection. We show that 3D NLTE successfully solves the ionisation and excitation balance for the RGB star HD 122563 that cannot be achieved by 1D LTE or 1D NLTE modelling. For HD 84937 and HD 140283, the ionisation balance is satisfied, however, the resonance Mn I triplet lines still show somewhat lower abundances compared to the high-excitation lines. Our results for the benchmark stars confirm that 1D LTE modelling leads to significant systematic biases in Mn abundances across the full wavelength range from the blue to the IR. We also produce a list of Mn lines that are not significantly biased by 3D and can be reliably, within the 0.1 dex uncertainty, modelled in 1D NLTE.

==> 4500_1.5_CH.tex <==
\begin{table*}
  \begin{center}
    \caption{NLTE abundance corrections for the MARCS models with $\teff = 4500$ K and $\log g = 1.5$ dex. See Fig. 9 in the main text.}
\setlength{\tabcolsep}{0.02\linewidth}
\begin{tabular}{c c c c c}
\hline
\noalign{\smallskip}
$\lambda \ [\AA]$ & [Fe/H] & CH excl. & CH0 excl. & CH/CH0 incl.  \\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
4030                           & 0                              & 0.157                          & 0.176                          & 0.153                           \\ 
4033                           & -1                             & 0.212                          & 0.236                          & 0.222                           \\ 
4034                           & -2                             & 0.378                          & 0.434                          & 0.426                           \\ 
                               & -3                             & 0.473                          & 0.483                          & 0.477                           \\ 
                               & 0                              & 0.198                          & 0.173                          & 0.156                           \\ 
4783                           & -1                             & 0.189                          & 0.214                          & 0.203                           \\ 
4823                           & -2                             & 0.333                          & 0.366                          & 0.358                           \\ 
                               & -3                             & 0.452                          & 0.462                          & 0.456                           \\ 
6013                           & 0                              & 0.203                          & 0.184                          & 0.174                           \\ 
6016                           & -1                             & 0.304                          & 0.288                          & 0.277                           \\ 
6021                           & -2                             & 0.372                          & 0.370                          & 0.364                           \\ 
                               & -3                             & 0.382                          & 0.396                          & 0.392                           \\ 
                               & 0                              & -0.013                         & -0.014                         & -0.013                          \\ 
3488                           & -1                             & -0.035                         & -0.035                         & -0.035                          \\ 
                               & -2                             & -0.078                         & -0.079                         & -0.079                          \\ 
                               & -3                             & 0.076                          & 0.074                          & 0.074                           \\ 
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\label{tableN1}
\end{table*}


==> 4500_1.5_k.tex <==
\begin{table*}
  \begin{center}
    \caption{NLTE abundance corrections for the MARCS models with $\teff = 4500$ K and $\log g = 1.5$ dex. See Fig. 10 in the main text.}
\setlength{\tabcolsep}{0.02\linewidth}
\begin{tabular}{c c c c}
\hline
\noalign{\smallskip}
$\lambda \ [\AA]$ & [Fe/H] & reference atom & no Kaulakys  \\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
4030                           & 0                              & 0.138                          & 0.153                           \\ 
4033                           & -1                             & 0.223                          & 0.222                           \\ 
4034                           & -2                             & 0.401                          & 0.426                           \\ 
                               & -3                             & 0.396                          & 0.477                           \\ 
                               & 0                              & 0.132                          & 0.156                           \\ 
4783                           & -1                             & 0.225                          & 0.203                           \\ 
4823                           & -2                             & 0.383                          & 0.358                           \\ 
                               & -3                             & 0.438                          & 0.456                           \\ 
6013                           & 0                              & 0.168                          & 0.174                           \\ 
6016                           & -1                             & 0.292                          & 0.277                           \\ 
6021                           & -2                             & 0.416                          & 0.364                           \\ 
                               & -3                             & 0.442                          & 0.392                           \\ 
                               & 0                              & -0.012                         & -0.013                          \\ 
3488                           & -1                             & -0.035                         & -0.035                          \\ 
                               & -2                             & -0.078                         & -0.079                          \\ 
                               & -3                             & 0.075                          & 0.074                           \\ 
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\label{tableN3}
\end{table*}


==> 6000_4.0_CH.tex <==
\begin{table*}
  \begin{center}
        \caption{NLTE abundance corrections for the MARCS models with $\teff = 6000$ K and $\log g = 4.0$ dex. See Fig. 9 in the main text.}

\setlength{\tabcolsep}{0.02\linewidth}
\begin{tabular}{c c c c c}
\hline
\noalign{\smallskip}
$\lambda \ [\AA]$ & [Fe/H] & CH excl. & CH0 excl. & CH/CH0 incl.  \\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
4030                           & 0                              & 0.043                          & 0.078                          & 0.042                           \\ 
4033                           & -1                             & -0.043                         & 0.002                          & -0.033                          \\ 
4034                           & -2                             & 0.124                          & 0.183                          & 0.113                           \\ 
                               & -3                             & 0.469                          & 0.529                          & 0.481                           \\ 
                               & 0                              & 0.002                          & 0.038                          & 0.014                           \\ 
4783                           & -1                             & 0.135                          & 0.186                          & 0.154                           \\ 
4823                           & -2                             & 0.272                          & 0.308                          & 0.274                           \\ 
                               & -3                             & 0.315                          & 0.354                          & 0.317                           \\ 
6013                           & 0                              & 0.123                          & 0.109                          & 0.090                           \\ 
6016                           & -1                             & 0.220                          & 0.226                          & 0.205                           \\ 
6021                           & -2                             & 0.280                          & 0.341                          & 0.322                           \\ 
                               & -3                             & 0.288                          & 0.395                          & 0.378                           \\ 
                               & 0                              & -0.017                         & -0.017                         & -0.016                          \\ 
3488                           & -1                             & -0.082                         & -0.080                         & -0.079                          \\ 
                               & -2                             & -0.038                         & -0.041                         & -0.040                          \\ 
                               & -3                             & 0.098                          & 0.093                          & 0.093                           \\ 
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\label{tableN2}
\end{table*}


==> 6000_4.0_k.tex <==
\begin{table*}
  \begin{center}
    \caption{NLTE abundance corrections for the MARCS models with $\teff = 6000$ K and $\log g = 4.0$ dex. See Fig. 10 in the main text.}
\setlength{\tabcolsep}{0.02\linewidth}
\begin{tabular}{c c c c}
\hline
\noalign{\smallskip}
$\lambda \ [\AA]$ & [Fe/H] & reference atom & no Kaulakys  \\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
4030                           & 0                              & 0.029                          & 0.042                           \\ 
4033                           & -1                             & -0.015                         & -0.033                          \\ 
4034                           & -2                             & 0.078                          & 0.113                           \\ 
                               & -3                             & 0.423                          & 0.481                           \\ 
                               & 0                              & 0.013                          & 0.014                           \\ 
4783                           & -1                             & 0.118                          & 0.154                           \\ 
4823                           & -2                             & 0.236                          & 0.274                           \\ 
                               & -3                             & 0.292                          & 0.317                           \\ 
6013                           & 0                              & 0.048                          & 0.090                           \\ 
6016                           & -1                             & 0.134                          & 0.205                           \\ 
6021                           & -2                             & 0.269                          & 0.322                           \\ 
                               & -3                             & 0.344                          & 0.378                           \\ 
                               & 0                              & -0.016                         & -0.016                          \\ 
3488                           & -1                             & -0.079                         & -0.079                          \\ 
                               & -2                             & -0.040                         & -0.040                          \\ 
                               & -3                             & 0.093                          & 0.093                           \\ 
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\label{table}
\end{table*}


==> tab1.tex <==
%
\begin{table}
\begin{minipage}{\linewidth}
\renewcommand{\footnoterule}{} 
\caption{Parameters of lines used for abundance calculation.}
 \label{lines}     
\begin{center}
\begin{tabular}{lrrlccc}
\noalign{\smallskip}\hline\noalign{\smallskip}  ~~~~~~$\lambda$ & M &
$N_{\rm HFS}$ & $\Elow$ & Lower & Upper & $\log gf$ \\
     ~~~~[\AA] &  &  & [eV] & level & level &   \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
  3488.68  &  -- &  3  &  1.85  &  \Mn{a}{5}{D}{ }{1}   & \Mn{z}{5}{P}{o}{1}    &  --0.937 \\
  3496.81  &  -- &  2  &  1.83  &  \Mn{a}{5}{D}{ }{2}   & \Mn{z}{5}{P}{o}{3}    &  --1.779 \\
  3497.53  &  -- &  3  &  1.85  &  \Mn{a}{5}{D}{ }{1}   & \Mn{z}{5}{P}{o}{2}    &  --1.418 \\
%                      
  4018.10   &  9  & 5  &  2.12  &  \Mn{a}{6}{D}{ }{9/2} & \Mn{z}{6}{D}{o}{7/2}  &  --0.311 \\
  4030.76   &  4  & 5  &  0.00  &  \Mn{a}{6}{S}{ }{5/2} & \Mn{z}{6}{P}{o}{7/2}  &  --0.497 \\
  4033.07   &  4  & 4  &  0.00  &  \Mn{a}{6}{S}{ }{5/2} & \Mn{z}{6}{P}{o}{5/2}  &  --0.647 \\
  4034.49   &  4  & 3  &  0.00  &  \Mn{a}{6}{S}{ }{5/2} & \Mn{z}{6}{P}{o}{3/2}  &  --0.843 \\
%  
  4055.54   &  9  & 4  &  2.14  &  \Mn{a}{6}{D}{ }{7/2} & \Mn{z}{6}{D}{o}{7/2}   & --0.077  \\
  4070.28   &  9  & 3  &  2.19  &  \Mn{a}{6}{D}{ }{1/2} & \Mn{z}{6}{D}{o}{1/2}   & --1.039  \\
  4451.58   &  24 & 3  &  2.89  &  \Mn{a}{4}{D}{ }{7/2} & \Mn{z}{4}{D}{o}{7/2}   &   0.278  \\
  4498.90   &  24 & 1  &  2.94  &  \Mn{a}{4}{D}{ }{2/2} & \Mn{z}{4}{D}{o}{5/2}   &   0.343  \\
  4502.22   &  24 & 2  &  2.92  &  \Mn{a}{4}{D}{ }{5/2} & \Mn{z}{4}{D}{o}{7/2}   & --0.345  \\
%                      
  4754.03  &  18 & 5  &  2.27  &  \Mn{z}{8}{P}{o}{5/2} & \Mn{e}{8}{S}{ }{7/2} &  --0.086 \\  
  4761.52  &  23 & 4  &  2.94  &  \Mn{a}{4}{D}{ }{1/2} & \Mn{z}{4}{F}{o}{3/2} &  --0.138 \\  
  4762.37  &  23 & 5  &  2.88  &  \Mn{a}{4}{D}{ }{7/2} & \Mn{z}{4}{F}{o}{9/2} &    0.425 \\  
  4765.86  &  23 & 3  &  2.93  &  \Mn{a}{4}{D}{ }{3/2} & \Mn{z}{4}{F}{o}{5/2} &  --0.080 \\  
  4766.42  &  23 & 4  &  2.91  &  \Mn{a}{4}{D}{ }{5/2} & \Mn{z}{4}{F}{o}{7/2} &    0.100 \\  
  4783.42  &  18 & 5  &  2.29  &  \Mn{z}{8}{P}{o}{7/2} & \Mn{e}{8}{S}{ }{7/2} &    0.042 \\  
  4823.51  &  18 & 6  &  2.31  &  \Mn{z}{8}{P}{o}{9/2} & \Mn{e}{8}{S}{ }{7/2} &    0.144 \\  
%  
  5004.89  &  22 & 4  &  2.91  &  \Mn{a}{4}{D}{ }{5/2} & \Mn{z}{6}{F}{o}{7/2} &  --1.630 \\  
  5117.93  &  39 & 3  &  3.12  &  \Mn{a}{4}{G}{ }{5/2} & \Mn{z}{4}{F}{o}{3/2} &  --1.140 \\  
  5255.31  &  39 & 6  &  3.12  &  \Mn{a}{4}{G}{ }{11/2}& \Mn{z}{4}{F}{o}{9/2} &  --0.763 \\  
  5394.67  &  2  & 6  &  0.00  &  \Mn{a}{6}{S}{ }{5/2} & \Mn{z}{8}{P}{o}{7/2} &  --3.503 \\  
  5407.42  &  8  & 10 &  2.13  &  \Mn{a}{6}{D}{ }{7/2} & \Mn{y}{6}{P}{o}{7/2} &  --1.743 \\  
  5420.35  &  8  & 9  &  2.13  &  \Mn{a}{6}{D}{ }{7/2} & \Mn{y}{6}{P}{o}{5/2} &  --1.462 \\  
  5432.54  &  2  & 5  &  0.00  &  \Mn{a}{6}{S}{ }{5/2} & \Mn{z}{8}{P}{o}{5/2} &  --3.795 \\  
  5470.63  &  4  & 8  &  2.15  &  \Mn{a}{6}{D}{ }{5/2} & \Mn{y}{6}{P}{o}{5/2} &  --1.702 \\  
%  
  5516.77  &  8  & 8  &  2.17  &  \Mn{a}{6}{D}{ }{3/2} & \Mn{y}{6}{P}{o}{3/2} &  --1.847 \\  
  5537.75  &  4  & 5  &  2.18  &  \Mn{a}{6}{D}{ }{1/2} & \Mn{y}{6}{P}{o}{3/2} &  --2.017 \\  
  6013.49  &  32 & 6  &  3.06  &  \Mn{z}{6}{P}{o}{3/2} & \Mn{e}{6}{S}{ }{5/2} &  --0.251 \\  
  6016.64  &  32 & 6  &  3.06  &  \Mn{z}{6}{P}{o}{5/2} & \Mn{e}{6}{S}{ }{5/2} &  --0.216 \\  
  6021.79  &  32 & 6  &  3.06  &  \Mn{z}{6}{P}{o}{7/2} & \Mn{e}{6}{S}{ }{5/2} &    0.034 \\  
%
% & 15159.
% & 15217.
% & 15262.
%
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular}
\end{center}
\end{minipage}
\end{table}



==> tab2.tex <==
%
\begin{table}
\begin{minipage}{\linewidth}
\renewcommand{\footnoterule}{} 
\caption{Parameters of 3D convective and 1D hydrostatic model atmospheres. In the 1D LTE radiative transfer calculations with MARCS models, we assume $\Vmic = 1$.}
\label{3dmodels}     
\begin{center}
\begin{tabular}{l l c c c c}
\noalign{\smallskip}\hline\noalign{\smallskip} No. & Name & $\teff$ & logg & $\feh$ &   \\
  & & K & dex & dex & \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
1 & Sun         & 5777  & 4.4  &  ~~0.0   &   \\
2 & HD 84937    & 6400  & 4.0  & $-$2.0   &   \\
3 & HD 140283   & 5750  & 3.7  & $-$2.5   &   \\
4 & HD 122563   & 4600  & 1.6  & $-$2.5   &   \\
\noalign{\smallskip}\hline\noalign{\smallskip}
% 
%5 & & 6500  & 4.0  & ~~0.0    &   \\
5 & Sub-solar metallicity dwarf & 6500  & 4.0  & $-$1.0   &   \\
6 & Metal-poor dwarf & 6500  & 4.0  & $-$2.0   &   \\
%
%8 & Metar-rich giant & 4500  & 2.0  & ~~0.0    &   \\
7 & Sub-solar metallicity giant & 4500  & 2.0  & $-$1.0   &   \\
8 & Metal-poor giant & 4500  & 2.0  & $-$2.0   &   \\
%
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular}
\end{center}
\end{minipage}
\end{table}



==> tables_H.tex <==
\begin{table}
\renewcommand{\tabcolsep}{4.5pt}
\caption{Scattering channels correlated to MgH molecular $^5\Sigma^+$ states, asymptotic energies ($J$-average experimental values taken from NIST) with respect to the ground state and electronic bound energies with respect to the ionization limit $\rm{Mn^+(3d^54s\,^5S) + H}$.}
\label{tab:states_MnH}
\begin{center}
\begin{tabular}{llcc}
j & Scattering channels & Asymptotic & Bound\\
  &                     & energy (eV)& energy (eV)\\
\noalign{\smallskip}\hline\noalign{\smallskip} 
 1 & $\rm{Mn(3d^54s^2 \,\,a^6S ) + H}$        & 0.000000 & -8.60854\\
 2 & $\rm{Mn(3d^64s   \,\,a^6D ) + H}$        & 2.145077 & -6.46346\\
 3 & $\rm{Mn(3d^64s   \,\,a^4D ) + H}$        & 2.914772 & -5.69377\\
 4 & $\rm{Mn(3d^54s4p \,\,z^6P^{\circ}) + H}$ & 3.073870 & -5.53467\\
 5 & $\rm{Mn(3d^54s^2 \,\,a^4G ) + H}$        & 3.134155 & -5.47438\\
 6 & $\rm{Mn(3d^54s^2 \,\,b^4D ) + H}$        & 3.768363 & -4.84018\\
 7 & $\rm{Mn(3d^54s4p \,\,z^4P^{\circ}) + H}$ & 3.849324 & -4.75921\\
 8 & $\rm{Mn(3d^54s4p \,\,y^6P^{\circ}) + H}$ & 4.430886 & -4.17765\\
 9 & $\rm{Mn(3d^64s   \,\,b^4G ) + H}$    & 4.663140 & -3.94540\\
10 & $\rm{Mn(3d^54s5s \,\,e^6S ) + H}$    & 5.133436 & -3.47510\\
11 & $\rm{Mn(3d^54s4d \,\,e^6D ) + H}$    & 5.853606 & -2.75493\\
12 & $\rm{Mn(3d^54s5p \,\,w^6P^{\circ}) + H}$ & 5.897434 & -2.71110\\
13 & $\rm{Mn(3d^54s4p \,\,y^6F^{\circ}) + H}$ & 5.972531 & -2.63601\\
14 & $\rm{Mn(3d^54s5s \,\,f^6S ) + H}$     & 6.126726 & -2.48181\\
15 & $\rm{Mn(3d^54s5s \,\,e^4S ) + H}$     & 6.148568 & -2.45997\\
16 & $\rm{Mn(3d^54s4p \,\,v^6P^{\circ}) + H}$ & 6.196287 & -2.41225\\
17 & $\rm{Mn(3d^54s4p \,\,z^4H^{\circ}) + H}$ & 6.209216 & -2.39932\\
18 & $\rm{Mn(3d^54s4p \,\,y^4F^{\circ}) + H}$ & 6.243758 & -2.36478\\
19 & $\rm{Mn(3d^54s4p \,\,x^6F^{\circ}) + H}$ & 6.328611 & -2.27993\\
20 & $\rm{Mn(3d^54s6s \,\,g^6S ) + H}$     & 6.311380 & -2.29716\\
21 & $\rm{Mn(3d^54s4p \,\,x^4P^{\circ}) + H}$ & 6.371961 & -2.23658\\
22 & $\rm{Mn(3d^54s4p \,\,u^6P^{\circ}) + H}$ & 6.466860 & -2.14168\\
23 & $\rm{Mn(3d^54s5d \,\,f^6D ) + H}$     & 6.537766 & -2.07077\\
24 & $\rm{Mn(3d^54s4f \,\,w^6F^{\circ}) + H}$ & 6.568422 & -2.04012\\
25 & $\rm{Mn(3d^54s6p \,\,t^6P^{\circ}) + H}$ & 6.606162 & -2.00238\\
26 & $\rm{Mn(3d^54s7s \,\,h^6S ) + H}$     & 6.752220 & -1.85632\\
27 & $\rm{Mn(3d^54s4d \,\,g^6D ) + H}$     & 6.812434 & -1.79610\\
28 & $\rm{Mn(3d^54s5p \,\,w^4P^{\circ}) + H}$ & 6.868987 & -1.73955\\
29 & $\rm{Mn(3d^54s5f \,\,v^6F^{\circ}) + H}$ & 6.880172 & -1.72837\\
30 & $\rm{Mn(3d^54s7p \,\,r^6P^{\circ}) + H}$ & 6.880244 & -1.72829\\
31 & $\rm{Mn(3d^54s6d \,\,h^6D ) + H}$        & 6.904357 & -1.70418\\
32 & $\rm{Mn(3d^54s5p \,\,t^4P^{\circ}) + H}$ & 6.934452 & -1.67409\\
33 & $\rm{Mn(3d^54s5p \,\,s^6P^{\circ}) + H}$ & 6.944067 & -1.66447\\
34 & $\rm{Mn(3d^65s   \,\,i^6D ) + H}$        & 6.989790 & -1.61875\\
35 & $\rm{Mn(3d^54s6f \,\,u^6F^{\circ}) + H}$ & 7.050626 & -1.55791\\
36 & $\rm{Mn(3d^54s8p \,\,q^6P^{\circ}) + H}$ & 7.058384 & -1.55016\\
37 & $\rm{Mn(3d^54s4p \,\,v^4P^{\circ}) + H}$ & 7.116923 & -1.49162\\
38 & $\rm{Mn(3d^54s7f \,\,t^6F^{\circ}) + H}$ & 7.153545 & -1.45499\\
39 & $\rm{Mn(3d^54s9p \,\,p^6P^{\circ}) + H}$ & 7.156234 & -1.45230\\
40 & $\rm{Mn(3d^54s10p\,\,o^6P^{\circ}) + H}$ & 7.220870 & -1.38767\\
41 & $\rm{Mn(3d^54s11p\,\, ^6P^{\circ}) + H}$ & 7.265446 & -1.34309\\
42 & $\rm{Mn(3d^54s12p\,\, ^6P^{\circ}) + H}$ & 7.297423 & -1.31112\\
43 & $\rm{Mn(3d^54s13p\,\, ^6P^{\circ}) + H}$ & 7.321116 & -1.28742\\
44 & $\rm{Mn(3d^54s14p\,\, ^6P^{\circ}) + H}$ & 7.339133 & -1.26941\\
45 & $\rm{Mn(3d^54s15p\,\, ^6P^{\circ}) + H}$ & 7.351767 & -1.25677\\
46 & $\rm{Mn(3d^54s16p\,\, ^6P^{\circ}) + H}$ & 7.364333 & -1.24421\\
47 & $\rm{Mn(3d^54s17p\,\, ^6P^{\circ}) + H}$ & 7.373379 & -1.23516\\
48 & $\rm{Mn(3d^54s18p\,\, ^6P^{\circ}) + H}$ & 7.380681 & -1.22786\\
49 & $\rm{Mn(3d^54s19p\,\, ^6P^{\circ}) + H}$ & 7.386776 & -1.22176\\
50 & $\rm{Mn(3d^54s20p\,\, ^6P^{\circ}) + H}$ & 7.391888 & -1.21665\\
\noalign{\smallskip}\hline\noalign{\smallskip}            
\end{tabular}                                             
\end{center}                                              
\end{table}                                               
                                                          
\begin{table}                                             
\renewcommand{\tabcolsep}{4.5pt}                          
\begin{center}                                            
\begin{tabular}{llcc}                                      
j & Scattering channel  & Asymptotic  & Bound\\                  
  &                     & energy (eV) & energy (eV)\\                  
\noalign{\smallskip}\hline\noalign{\smallskip}            
51 & $\rm{Mn(3d^54s21p\,\, ^6P^{\circ}) + H}$ & 7.396210 & -1.21233\\
52 & $\rm{Mn(3d^54s22p\,\, ^6P^{\circ}) + H}$ & 7.399904 & -1.20864\\
53 & $\rm{Mn(3d^54s23p\,\, ^6P^{\circ}) + H}$ & 7.403078 & -1.20546\\
54 & $\rm{Mn(3d^54s24p\,\, ^6P^{\circ}) + H}$ & 7.405828 & -1.20271\\
55 & $\rm{Mn(3d^54s25p\,\, ^6P^{\circ}) + H}$ & 7.408231 & -1.20031\\
56 & $\rm{Mn(3d^54s26p\,\, ^6P^{\circ}) + H}$ & 7.410336 & -1.19820\\
57 & $\rm{Mn(3d^54s27p\,\, ^6P^{\circ}) + H}$ & 7.412199 & -1.19634\\
58 & $\rm{Mn(3d^54s28p\,\, ^6P^{\circ}) + H}$ & 7.413848 & -1.19469\\
59 & $\rm{Mn(3d^54s29p\,\, ^6P^{\circ}) + H}$ & 7.415318 & -1.19322\\
60 & $\rm{Mn(3d^54s30p\,\, ^6P^{\circ}) + H}$ & 7.416628 & -1.19191\\
61 & $\rm{Mn(3d^54s31p\,\, ^6P^{\circ}) + H}$ & 7.417802 & -1.19074\\
62 & $\rm{Mn(3d^54s32p\,\, ^6P^{\circ}) + H}$ & 7.418876 & -1.18966\\
63 & $\rm{Mn(3d^54s33p\,\, ^6P^{\circ}) + H}$ & 7.419839 & -1.18870\\
64 & $\rm{Mn(3d^54s34p\,\, ^6P^{\circ}) + H}$ & 7.420701 & -1.18784\\
65 & $\rm{Mn(3d^54s35p\,\, ^6P^{\circ}) + H}$ & 7.421504 & -1.18704\\
66 & $\rm{Mn(3d^54s36p\,\, ^6P^{\circ}) + H}$ & 7.422245 & -1.18629\\
67 & $\rm{Mn(3d^54s37p\,\, ^6P^{\circ}) + H}$ & 7.422891 & -1.18565\\
68 & $\rm{Mn(3d^54s38p\,\, ^6P^{\circ}) + H}$ & 7.423498 & -1.18504\\
69 & $\rm{Mn(3d^54s39p\,\, ^6P^{\circ}) + H}$ & 7.424055 & -1.18448\\
70 & $\rm{Mn(3d^54s40p\,\, ^6P^{\circ}) + H}$ & 7.424578 & -1.18396\\
71 & $\rm{Mn(3d^54s41p\,\, ^6P^{\circ}) + H}$ & 7.425049 & -1.18349\\
72 & $\rm{Mn^+(3d^54s\,^5S) + H^-}$           & 7.854539 & -0.754\\
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular}
\end{center}
\end{table}

\begin{table}
\renewcommand{\tabcolsep}{4.5pt}
\caption{Scattering channels correlated to MgH$^+$ molecular $^6\Sigma^+$ states, asymptotic energies ($J$-average experimental values taken from NIST with respect to the ground state and electronic bound energies with respect to the ionization limit $\rm{Mn^{2+}(3d^5\,^6S) + H}$.}
\label{tab:states_MnH+}
\begin{center}
\begin{tabular}{llcc}
j & Scattering channel  & Asymptotic & Bound\\
  &                     & energy (eV)& energy (eV)\\
\noalign{\smallskip}\hline\noalign{\smallskip} 
 1 & $\rm{Mn^+(3d^54s\,\,a^7S ) + H}$        & 0.000000 & -15.6400\\
 2 & $\rm{Mn^+(3d^54s\,\,a^5S ) + H}$        & 1.174501 & -14.4655\\
 3 & $\rm{Mn^+(3d^6  \,\,a^5D ) + H}$        & 1.808479 & -13.8315\\
 4 & $\rm{Mn^+(3d^54s\,\,a^5G ) + H}$     & 3.418429 & -12.2216\\
 5 & $\rm{Mn^+(3d^54s\,\,b^5D ) + H}$        & 4.070230 & -11.5698\\
 6 & $\rm{Mn^+(3d^54p\,\,z^7P^{\circ}) + H}$ & 4.787521 & -10.8525\\
 7 & $\rm{Mn^+(3d^54p\,\,z^5P^{\circ}) + H}$ & 5.386607 & -10.2534\\
 8 & $\rm{Mn^+(3d^54p\,\,z^5H^{\circ}) + H}$ & 8.145176 & -7.49481\\
 9 & $\rm{Mn^+(3d^54p\,\,z^5F^{\circ}) + H}$ & 8.267108 & -7.37288\\
10 & $\rm{Mn^+(3d^54p\,\,y^5P^{\circ}) + H}$ & 8.476972 & -7.16302\\
11 & $\rm{Mn^+(3d^54p\,\,y^5F^{\circ}) + H}$ & 8.734600 & -6.90539\\
12 & $\rm{Mn^+(3d^54p\,\,x^5P^{\circ}) + H}$ & 8.845407 & -6.79458\\
13 & $\rm{Mn^+(3d^55s\,\,e^7S ) + H}$     & 9.244271 & -6.39572\\
14 & $\rm{Mn^+(3d^55s\,\,e^5S ) + H}$     & 9.469252 & -6.17074\\
15 & $\rm{Mn^+(3d^54d\,\,e^7D ) + H}$     & 9.863794 & -5.77620\\
16 & $\rm{Mn^+(3d^54p\,\,x^5F^{\circ}) + H}$ & 10.16684 & -5.47314\\
17 & $\rm{Mn^+(3d^54d\,\,e^5D ) + H}$     & 10.18466 & -5.45532\\
18 & $\rm{Mn^+(3d^55p\,\,x^7P^{\circ}) + H}$ & 10.66097 & -4.97902\\
19 & $\rm{Mn^+(3d^55p\,\,v^5P^{\circ}) + H}$ & 11.05872 & -4.58127\\
20 & $\rm{Mn^+(3d^56s\,\,f^7S ) + H}$     & 12.11680 & -3.52319\\
21 & $\rm{Mn^+(3d^56s\,\,f^5S ) + H}$      & 12.20133 & -3.43865\\
22 & $\rm{Mn^+(3d^54f\,\,z^7F^{\circ}) + H}$ & 12.20296 & -3.43702\\
23 & $\rm{Mn^+(3d^54f\,\,e^5F^{\circ}) + H}$ & 12.20797 & -3.43202\\
24 & $\rm{Mn^+(3d^55d\,\,f^7D ) + H}$      & 12.38580 & -3.25419\\
25 & $\rm{Mn^+(3d^55d\,\,f^5D ) + H}$      & 12.48374 & -3.15624\\
26 & $\rm{Mn^+(3d^55s\,\,e^5G ) + H}$     & 12.58296 & -3.05702\\
27 & $\rm{Mn^+(3d^54d\,\,e^5I ) + H}$     & 13.20636 & -2.43362\\
28 & $\rm{Mn^+(3d^55s\,\,g^5D ) + H}$     & 13.25794 & -2.38204\\
29 & $\rm{Mn^+(3d^57s\,\,g^7S ) + H}$     & 13.40594 & -2.23404\\
30 & $\rm{Mn^+(3d^55f\,\,y^7F^{\circ}) + H}$ & 13.44114 & -2.19885\\
31 & $\rm{Mn^+(3d^55f\,\,f^5F^{\circ}) + H}$ & 13.44490 & -2.19509\\
32 & $\rm{Mn^+(3d^57s\,\,g^5S ) + H}$     & 13.44576 & -2.19423\\
33 & $\rm{Mn^+(3d^55g\,\,e^7G ) + H}$     & 13.45920 & -2.18079\\
34 & $\rm{Mn^+(3d^55g\,\,f^5G ) + H}$        & 13.45925 & -2.18074\\
35 & $\rm{Mn^+(3d^56d\,\,g^7D ) + H}$     & 13.54475 & -2.09524\\
36 & $\rm{Mn^+(3d^55p\,\,s^5F^{\circ}) + H}$ & 14.09071 & -1.54927\\
37 & $\rm{Mn^+(3d^58s\,\,h^7S ) + H}$     & 14.09672 & -1.54327\\
38 & $\rm{Mn^+(3d^56f\,\,x^7F^{\circ}) + H}$ & 14.11439 & -1.52559\\
39 & $\rm{Mn^+(3d^56g\,\,f^7G ) + H}$     & 14.12574 & -1.51425\\
40 & $\rm{Mn^+(3d^56g\,\,g^5G ) + H}$     & 14.12579 & -1.51420\\
41 & $\rm{Mn^+(3d^56f\,\,g^5F^{\circ}) + H}$ & 14.13750 & -1.50249\\
42 & $\rm{Mn^+(3d^57d\,\,h^5D ) + H}$     & 14.25117 & -1.38882\\
43 & $\rm{Mn^{2+}(3d^5\,^6S) + H^-}$         & 14.88599 & -0.754\\
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular}
\end{center}
\end{table}


==> tables_ph.tex <==
\begin{table*}[h]
\caption{LS terms of the target \ion{Mn}{ii} ion included in the close 
coupling expansion.}
\label{fe2target}    
\centering          
\begin{tabular}[scriptsize]{llllllllllll}     % 7 columns 
\hline\hline       
Configuration&Term&\multicolumn{2}{c}{Energy (Ryd)} 
& Configuration&Term&\multicolumn{2}{c}{Energy (Ryd)}&  Configuration&Term&\multicolumn{2}{c}{Energy (Ryd)}
\cr
 & & Theory & Exp. & & & Theory & Exp. & & & Theory & Exp. \cr
\\
\hline
3d$^5$($^6$S)4s &$^7$S    &0.0000 &0.0000  & 3d$^5$($^2$G)4s &$^3$G    &0.5430& 0.4508  & 3d$^5$($^4$D)4p &$^3$D$^o$ &0.7630& 0.6688  \cr
3d$^5$($^6$S)4s &$^5$S    &0.1048 &0.0863  & 3d$^5$($^4$F)4s &$^3$F    &0.5491& 0.4544  & 3d$^5$($^4$D)4p &$^3$F$^o$ &0.7678& 0.6720  \cr
3d$^6$  &     $^5$D       &0.1560 &0.1331  & 3d$^5$($^2$F)4s &$^1$F    &0.5495& 0.4290  & 3d$^5$($^2$I)4p &$^3$I$^o$ &0.7847& 0.7137  \cr
3d$^5$($^4$G)4s &$^5$G    &0.2983 &0.2513  & 3d$^5$($^2$H)4s &$^1$H    &0.5607& 0.4698  & 3d$^5$($^4$P)4p &$^3$S$^o$ &0.7881& 0.6735  \cr
3d$^6$       &$^3$H       &0.3230 &0.2793  & 3d$^5$($^2$F)4s &$^3$F    &0.5742& 0.4773  & 3d$^5$($^2$G)4s &$^1$G     &0.7973& 0.6620  \cr
3d$^6$       &$^3$P       &0.3358 &0.2764  & 3d$^5$($^2$G)4s &$^1$G    &0.5760& 0.4798  & 3d$^5$($^4$D)4p &$^3$P$^o$ &0.7976& 0.6907  \cr
3d$^5$($^4$P)4s &$^5$P    &0.3406 &0.2726  & 3d$^6$       &$^3$P       &0.5859& 0.4853  & 3d$^5$($^2$I)4p &$^1$H$^o$ &0.7978& 0.7209  \cr
3d$^6$       &$^3$F       &0.3436 &0.2882  & 3d$^6$       &$^3$F       &0.5929& 0.4900  & 3d$^5$($^2$I)4p &$^3$H$^o$ &0.8043& 0.7263  \cr
3d$^6$       &$^3$G       &0.3488 &0.3178  & 3d$^5$($^2$F)4s &$^1$F    &0.6204& 0.5081  & 3d$^5$(a $^2$D)4p&$^1$D$^o$ &0.8247& 0.7191  \cr
3d$^5$($^6$S)4p&$^7$P$^o$ &0.3564 &0.3518  & 3d$^5$($^2$S)4s &$^3$S    &0.6371& 0.5184  & 3d$^5$(a $^2$D)4p&$^3$F$^o$ &0.8259& 0.7260  \cr
3d$^5$($^4$D)4s &$^5$S    &0.3660 &0.2992  & 3d$^5$($^4$G)4p&$^5$G$^o$ &0.6402& 0.5878  & 3d$^5$($^2$I)4p &$^1$I$^o$ &0.8374& 0.7454  \cr
3d$^5$($^4$G)4s &$^3$G    &0.3828 &0.3027  & 3d$^6$       &$^1$G       &0.6486& 0.5425  & 3d$^5$(a $^2$F)4p&$^1$G$^o$ &0.8449& 0.7407  \cr
3d$^6$        &$^3$D      &0.4022 &0.3448  & 3d$^4$4s$^2$    &$^5$D    &0.6552& 0.5043  & 3d$^5$($^4$F)4p &$^5$G$^o$ &0.8508& 0.7475  \cr
3d$^6$       &$^1$I       &0.4043 &0.3528  & 3d$^5$($^4$G)4p&$^5$H$^o$ &0.6555& 0.5986  & 3d$^5$(a $^2$D)4p&$^3$P$^o$ &0.8524& 0.7409  \cr
3d$^5$($^4$P)4s &$^3$P    &0.4133 &0.3311  & 3d$^5$($^4$G)4p&$^5$F$^o$ &0.6680& 0.6077  & 3d$^5$($^2$F)4p &$^3$G$^o$ &0.8528& 0.7493  \cr
3d$^6$       &$^1$G       &0.4133 &0.3545  & 3d$^5$($^4$P)4p&$^5$D$^o$ &0.6839& 0.6102  & 3d$^5$($^4$F)4p &$^5$F$^o$ &0.8543& 0.7473  \cr
3d$^5$($^6$S)4p&$^5$P$^o$ &0.4331 &0.3959  & 3d$^5$($^4$P)4p&$^5$S$^o$ &0.6858& 0.6099  & 3d5.(a $^2$D)4p  &$^1$F$^o$ &0.8549& 0.7401  \cr
3d$^5$($^2$I)4s &$^3$I    &0.4373 &0.3754  & 3d$^5$($^4$G)4p&$^3$F$^o$ &0.6887& 0.6181  & 3d$^5$($^2$D)4p &$^3$D$^o$ &0.8591& 0.7447  \cr
3d$^5$($^4$D)4s &$^3$D    &0.4449 &0.3628  & 3d$^5$($^4$G)4p&$^3$H$^o$ &0.6925& 0.6181  & 3d$^5$($^4$F)4p &$^5$D$^o$ &0.8604& 0.7536  \cr
3d$^6$       &$^1$S       &0.4478 &0.3714  & 3d$^5$($^2$D)4s &$^3$D    &0.6977& 0.5702  & 3d$^5$(a $^2$F)4p&$^3$F$^o$ &0.8650& 0.7553  \cr
3d$^5$($^2$I)4s &$^1$I    &0.4720 &0.4038  & 3d$^5$($^4$P)4p&$^5$P$^o$ &0.7002& 0.6231  & 3d$^5$(a $^2$F)4p&$^3$D$^o$ &0.8673& 0.7541  \cr
3d$^5$($^4$F)4s &$^5$F    &0.4810 &0.3972  & 3d$^5$($^4$D)4p&$^5$F$^o$ &0.7185& 0.6419  & 3d$^5$(a $^2$G)4p&$^3$H$^o$ &0.8674& 0.7698  \cr
3d$^6$       &$^1$D       &0.4812 &0.3930  & 3d$^5$($^4$P)4p&$^3$P$^o$ &0.7193& 0.6301  & 3d$^5$($^4$F)4p &$^3$G$^o$ &0.8741& 0.7646  \cr
3d$^5$($^2$F)4s &$^3$F    &0.4965 &0.4074  & 3d$^5$($^2$D)4s &$^1$D    &0.7243& 0.5975  & 3d$^5$($^2$H)4p &$^3$I$^o$ &0.8824& 0.7805  \cr
3d$^5$($^2$D)4s &$^3$D    &0.4990 &0.3968  & 3d$^5$($^4$G)4p&$^3$G$^o$ &0.7289& 0.6427  & 3d$^5$(a $^2$D)4p&$^1$P$^o$ &0.8864& 0.7679  \cr
3d$^6$       &$^1$F       &0.5099 &0.4492  & 3d$^5$($^4$D)4p&$^5$P$^o$ &0.7335& 0.6501  & 3d$^5$($^2$H)4p &$^3$G$^o$ &0.8890& 0.7804  \cr
3d$^5$($^2$D)4s &$^1$D    &0.5254 &0.4274  & 3d$^5$($^4$D)4p&$^5$D$^o$ &0.7412& 0.6579  & 3d$^5$(a $^2$F)4p&$^1$D$^o$ &0.8973& 0.7779  \cr
3d$^5$($^2$H)4s &$^3$H    &0.5269 &0.4408  & 3d$^5$($^4$P)4p&$^3$D$^o$ &0.7431& 0.6459  & 3d$^5$($^2$I)4p &$^1$H$^o$ &0.9274& 0.7212  \cr
\hline                  
\end{tabular}
\end{table*}

\begin{table}
\caption{{\sc autostructure} configuration expansions for \ion{Mn}{ii}.\label{table:AUTOconfigs}}
\centering                          % used for centering table
\begin{tabular}{l}        % centered columns (1 columns)
Configuration expansion\\
\hline\hline
3d$^6$, 3d$^5$4s, 3d$^5$4p, 3d$^5$4d, 3d$^5$5s, 3d$^5$5p,
3d$^4$4s$^2$, \\
3d$^4$4s4p, 3d$^4$4s4d, 3d$^4$4p$^2$\\ 
\hline
$\lambda_{1s}=1.00000,$ 
$\lambda_{2s}=1.25438,$ 
$\lambda_{2p}=1.10633,$
$\lambda_{3s}=1.10274,$\\
$\lambda_{3p}=1.06738,$
$\lambda_{3d}=1.06340,$
$\lambda_{4s}=1.02844,$
$\lambda_{4p}=1.11707,$\\
$\lambda_{4d}=1.46349,$
$\lambda_{5s}= 1.00000,$
$\lambda_{5p}=1.00000$
\\
\hline                                   %inserts single line
\end{tabular}
\end{table}

